Algorithm 979: Recursive Algorithms for Dense Linear Algebra -- The ReLAPACK Collection

To exploit both memory locality and the full performance potential of highly tuned kernels, dense linear algebra libraries such as LAPACK commonly implement operations as blocked algorithms. However, to achieve next-to-optimal performance with such algorithms, significant tuning is required. On the other hand, recursive algorithms are virtually tuning free, and yet attain similar performance. In this paper, we first analyze and compare blocked and recursive algorithms in terms of performance, and then introduce ReLAPACK, an open-source library of recursive algorithms to seamlessly replace most of LAPACK's blocked algorithms. In many scenarios, ReLAPACK clearly outperforms reference LAPACK, and even improves upon the performance of optimizes libraries.

==> fullsource/Makefile <==
PDFLATEX = pdflatex -shell-escape -recorder

TARGET = main.pdf

TEXFILES = *.tex figures/*.tex

default: once

# internals below

TARGETSTEM = $(TARGET:.pdf=)

once: 
	$(PDFLATEX) $(TARGETSTEM)

twice:
	make once
	make once

figs:
	time make -j 4 -f $(TARGETSTEM).makefile

ffigs:
	time make -j 4 -f $(TARGETSTEM).makefile -B

bib:
	bibtex $(TARGETSTEM)

all:
	make once
	make figs
	make bib
	make once
	make ffigs
	make twice

bg:
	make once < /dev/null 2>&1 1> /dev/null &

check: $(TEXFILES)
	for file in $(TEXFILES); \
	do \
		aspell --lang=EN --mode=tex check $$file; \
	done

open:
	open $(TARGET)

clean:
	rm -rf $(TARGETSTEM).{blg,fls,aux,log,toc,pdf,lof,out,figlist,makefile,pyg} figures/externalized/*

